Designing and Training of Lightweight Neural Networks on Edge Devices using Early Halting in Knowledge Distillation

Automated feature extraction capability and significant performance of Deep Neural Networks (DNN) make them suitable for Internet of Things (IoT) applications. However, deploying DNN on edge devices becomes prohibitive due to the colossal computation, energy, and storage requirements. This paper presents a novel approach for designing and training lightweight DNN using large-size DNN. The approach considers the available storage, processing speed, and maximum allowable processing time to execute the task on edge devices. We present a knowledge distillation based training procedure to train the lightweight DNN to achieve adequate accuracy. During the training of lightweight DNN, we introduce a novel early halting technique, which preserves network resources; thus, speedups the training procedure. Finally, we present the empirically and real-world evaluations to verify the effectiveness of the proposed approach under different constraints using various edge devices.

==> c/0.2/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.6,0.6;
set ylabel 'Accuracy (\%)' offset 2.0;
set xlabel 'Regular DNN model' offset 0,0.5;
set xtics ('$\mathbf{M}_2$' 2,'$\mathbf{M}_4$' 5)
#set xtic rotate by -45 scale 0
set ytics ('\textbf{40}' 40, '\textbf{60}' 60, '\textbf{80}' 80, '\textbf{100}' 100) 
set grid
#set key horizontal
set key at 7.0,104.2 horizontal
#width -0.75 opaque box maxrow 1.2
set key samplen 1.5
set key width -1  
set boxwidth 0.24 relative
set style fill solid 0.9
plot [0.0:7.0][20:105] "final_out_d1" u ($1-0.78):2 w boxes fill pattern 2 lc rgb "#006400" lw 4 title '$\mathbf{M}^t$', "final_out_d1" u ($1-0.00):3 w boxes fill pattern 7 lc rgb "#FF0F00" lw 3 title '$\mathbf{M}^r$', "final_out_d1" u ($1+0.78):4 w boxes fill pattern 3 lc rgb "#0010FF" lw 3 title '$\mathbf{M}^s$'


==> c/0.2/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,1114){\makebox(0,0)[r]{\strut{}\textbf{40}}}%
      \csname LTb\endcsname%%
      \put(946,1634){\makebox(0,0)[r]{\strut{}\textbf{60}}}%
      \csname LTb\endcsname%%
      \put(946,2153){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(946,2673){\makebox(0,0)[r]{\strut{}\textbf{100}}}%
      \csname LTb\endcsname%%
      \put(1891,374){\makebox(0,0){\strut{}$\mathbf{M}_2$}}%
      \csname LTb\endcsname%%
      \put(3110,374){\makebox(0,0){\strut{}$\mathbf{M}_4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,1698){\rotatebox{-270}{\makebox(0,0){\strut{}Accuracy (\%)}}}%
      \put(2500,154){\makebox(0,0){\strut{}Regular DNN model}}%
      \csname LTb\endcsname%%
      \put(1820,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^t$}}%
      \csname LTb\endcsname%%
      \put(2609,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^r$}}%
      \csname LTb\endcsname%%
      \put(3398,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^s$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> c/0.2/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> c/0.2/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> c/0.4/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.6,0.6;
set ylabel 'Accuracy (\%)' offset 2.0;
set xlabel 'Regular DNN model' offset 0,0.5;
set xtics ('$\mathbf{M}_2$' 2,'$\mathbf{M}_4$' 5)
#set xtic rotate by -45 scale 0
set ytics ('\textbf{40}' 40, '\textbf{60}' 60, '\textbf{80}' 80, '\textbf{100}' 100) 
set grid
#set key horizontal
set key at 7.0,104.2 horizontal
#width -0.75 opaque box maxrow 1.2
set key samplen 1.5
set key width -1  
set boxwidth 0.24 relative
set style fill solid 0.9
plot [0.0:7.0][20:105] "final_out_d1" u ($1-0.78):2 w boxes fill pattern 2 lc rgb "#006400" lw 4 title '$\mathbf{M}^t$', "final_out_d1" u ($1-0.00):3 w boxes fill pattern 7 lc rgb "#FF0F00" lw 3 title '$\mathbf{M}^r$', "final_out_d1" u ($1+0.78):4 w boxes fill pattern 3 lc rgb "#0010FF" lw 3 title '$\mathbf{M}^s$'


==> c/0.4/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,1114){\makebox(0,0)[r]{\strut{}\textbf{40}}}%
      \csname LTb\endcsname%%
      \put(946,1634){\makebox(0,0)[r]{\strut{}\textbf{60}}}%
      \csname LTb\endcsname%%
      \put(946,2153){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(946,2673){\makebox(0,0)[r]{\strut{}\textbf{100}}}%
      \csname LTb\endcsname%%
      \put(1891,374){\makebox(0,0){\strut{}$\mathbf{M}_2$}}%
      \csname LTb\endcsname%%
      \put(3110,374){\makebox(0,0){\strut{}$\mathbf{M}_4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,1698){\rotatebox{-270}{\makebox(0,0){\strut{}Accuracy (\%)}}}%
      \put(2500,154){\makebox(0,0){\strut{}Regular DNN model}}%
      \csname LTb\endcsname%%
      \put(1820,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^t$}}%
      \csname LTb\endcsname%%
      \put(2609,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^r$}}%
      \csname LTb\endcsname%%
      \put(3398,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^s$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> c/0.4/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> c/0.4/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> c/0.6/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.6,0.6;
set ylabel 'Accuracy (\%)' offset 2.0;
set xlabel 'Regular DNN model' offset 0,0.5;
set xtics ('$\mathbf{M}_2$' 2,'$\mathbf{M}_4$' 5)
#set xtic rotate by -45 scale 0
set ytics ('\textbf{40}' 40, '\textbf{60}' 60, '\textbf{80}' 80, '\textbf{100}' 100) 
set grid
#set key horizontal
set key at 7.0,104.2 horizontal
#width -0.75 opaque box maxrow 1.2
set key samplen 1.5
set key width -1  
set boxwidth 0.24 relative
set style fill solid 0.9
plot [0.0:7.0][20:105] "final_out_d1" u ($1-0.78):2 w boxes fill pattern 2 lc rgb "#006400" lw 4 title '$\mathbf{M}^t$', "final_out_d1" u ($1-0.00):3 w boxes fill pattern 7 lc rgb "#FF0F00" lw 3 title '$\mathbf{M}^r$', "final_out_d1" u ($1+0.78):4 w boxes fill pattern 3 lc rgb "#0010FF" lw 3 title '$\mathbf{M}^s$'


==> c/0.6/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,1114){\makebox(0,0)[r]{\strut{}\textbf{40}}}%
      \csname LTb\endcsname%%
      \put(946,1634){\makebox(0,0)[r]{\strut{}\textbf{60}}}%
      \csname LTb\endcsname%%
      \put(946,2153){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(946,2673){\makebox(0,0)[r]{\strut{}\textbf{100}}}%
      \csname LTb\endcsname%%
      \put(1891,374){\makebox(0,0){\strut{}$\mathbf{M}_2$}}%
      \csname LTb\endcsname%%
      \put(3110,374){\makebox(0,0){\strut{}$\mathbf{M}_4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,1698){\rotatebox{-270}{\makebox(0,0){\strut{}Accuracy (\%)}}}%
      \put(2500,154){\makebox(0,0){\strut{}Regular DNN model}}%
      \csname LTb\endcsname%%
      \put(1820,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^t$}}%
      \csname LTb\endcsname%%
      \put(2609,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^r$}}%
      \csname LTb\endcsname%%
      \put(3398,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^s$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> c/0.6/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> c/0.6/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> c/0.8/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.6,0.6;
set ylabel 'Accuracy (\%)' offset 2.0;
set xlabel 'Regular DNN model' offset 0,0.5;
set xtics ('$\mathbf{M}_2$' 2,'$\mathbf{M}_4$' 5)
#set xtic rotate by -45 scale 0
set ytics ('\textbf{40}' 40, '\textbf{60}' 60, '\textbf{80}' 80, '\textbf{100}' 100) 
set grid
#set key horizontal
set key at 7.0,104.2 horizontal
#width -0.75 opaque box maxrow 1.2
set key samplen 1.5
set key width -1  
set boxwidth 0.24 relative
set style fill solid 0.9
plot [0.0:7.0][20:105] "final_out_d1" u ($1-0.78):2 w boxes fill pattern 2 lc rgb "#006400" lw 4 title '$\mathbf{M}^t$', "final_out_d1" u ($1-0.00):3 w boxes fill pattern 7 lc rgb "#FF0F00" lw 3 title '$\mathbf{M}^r$', "final_out_d1" u ($1+0.78):4 w boxes fill pattern 3 lc rgb "#0010FF" lw 3 title '$\mathbf{M}^s$'


==> c/0.8/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,1114){\makebox(0,0)[r]{\strut{}\textbf{40}}}%
      \csname LTb\endcsname%%
      \put(946,1634){\makebox(0,0)[r]{\strut{}\textbf{60}}}%
      \csname LTb\endcsname%%
      \put(946,2153){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(946,2673){\makebox(0,0)[r]{\strut{}\textbf{100}}}%
      \csname LTb\endcsname%%
      \put(1891,374){\makebox(0,0){\strut{}$\mathbf{M}_2$}}%
      \csname LTb\endcsname%%
      \put(3110,374){\makebox(0,0){\strut{}$\mathbf{M}_4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,1698){\rotatebox{-270}{\makebox(0,0){\strut{}Accuracy (\%)}}}%
      \put(2500,154){\makebox(0,0){\strut{}Regular DNN model}}%
      \csname LTb\endcsname%%
      \put(1820,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^t$}}%
      \csname LTb\endcsname%%
      \put(2609,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^r$}}%
      \csname LTb\endcsname%%
      \put(3398,2672){\makebox(0,0)[r]{\strut{}$\mathbf{M}^s$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> c/0.8/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> c/0.8/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> class_wise/m1/1_ <==
set terminal epslatex;
set output '1.tex'; 
set size .73,.5;
set xlabel '{\footnotesize Regularization Parameter \alpha}';
set ylabel '{\footnotesize Overall Accuracy of Symbols}' offset 3;
set pointsize 1;
set ytics 0.65,0.1,1.0
set xtics ('$10^{-3}' 1, '$10^{-2}' 2, '$10^{-1}' 3, '$10^{0}' 4, '$10^{1}' 5)
plot [][0.55:0.95] 'res2.txt' using 1:2 with linespoints lt 1 lc rgb "red" lw 1 pt 1 title '\footnotesize No hidden layer','res2.txt' using 1:3 with linespoints lt 2 lc rgb "blue" lw 1 pt 2 title '\footnotesize One hidden layer','res2.txt' using 1:4 with linespoints lt 3 lc rgb "black" lw 1 pt 3 title '\footnotesize Two hidden layers'


==> class_wise/m1/dbd/1 <==
set terminal epslatex;
set output '1.tex';
set size 0.5,0.5;
#set border 2 front lt black linewidth 1.000 dashtype solid
set boxwidth 0.4 absolute
set style fill solid 0.50 border lt -1
#set key horizontal
set grid
set key off
set pointsize 0.5
set style data boxplot
#set xtics border in scale 0,0  rotate  
#set xtics  offset -1,-1.5 norangelimit 
set xtics ('\large$\mathbf{h_1}$' 1, '\large$\mathbf{h_2}$' 2, '\large$\mathbf{h_3}$' 3, '\large$\mathbf{h_4}$' 4)
set ytics ('\textbf{80}'80,'\textbf{85}'85,'\textbf{90}'90,'\textbf{95}'95,'\textbf{100}'100)
set ylabel '\large\textbf{Accuracy}' offset 3.0
set xlabel '\large\textbf{Class labels}'
set yrange [ 80: 100 ]
x = 0.0
## Last datafile plotted: "silver.dat"
plot 'silver.dat' using (1):2 lc rgb "magenta" title "Still",'silver.dat' using (2):3 lc rgb "green"title "Walk", 'silver.dat' using (3):4 lc rgb "blue" title "Run", 'silver.dat' using (4):5 lc rgb "red" title "Bike"


==> class_wise/m1/dbd/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3600.00,2520.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(946,1103){\makebox(0,0)[r]{\strut{}\textbf{85}}}%
      \csname LTb\endcsname%%
      \put(946,1502){\makebox(0,0)[r]{\strut{}\textbf{90}}}%
      \csname LTb\endcsname%%
      \put(946,1901){\makebox(0,0)[r]{\strut{}\textbf{95}}}%
      \csname LTb\endcsname%%
      \put(946,2300){\makebox(0,0)[r]{\strut{}\textbf{100}}}%
      \csname LTb\endcsname%%
      \put(1382,484){\makebox(0,0){\strut{}\large$\mathbf{h_1}$}}%
      \csname LTb\endcsname%%
      \put(1888,484){\makebox(0,0){\strut{}\large$\mathbf{h_2}$}}%
      \csname LTb\endcsname%%
      \put(2393,484){\makebox(0,0){\strut{}\large$\mathbf{h_3}$}}%
      \csname LTb\endcsname%%
      \put(2899,484){\makebox(0,0){\strut{}\large$\mathbf{h_4}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(594,1502){\rotatebox{-270}{\makebox(0,0){\strut{}\large\textbf{Accuracy}}}}%
      \put(2140,154){\makebox(0,0){\strut{}\large\textbf{Class labels}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> class_wise/m1/dbm/1 <==
set terminal epslatex;
set output '1.tex';
set size 0.5,0.5;
#set border 2 front lt black linewidth 1.000 dashtype solid
set boxwidth 0.4 absolute
set style fill solid 0.50 border lt -1
#set key horizontal
set grid
set key off
set pointsize 0.5
set style data boxplot
#set xtics border in scale 0,0  rotate  
#set xtics  offset -1,-1.5 norangelimit 
set xtics ('\large$\mathbf{f_1}$' 1, '\large$\mathbf{f_2}$' 2, '\large$\mathbf{f_3}$' 3, '\large$\mathbf{f_4}$' 4)
set ytics ('\textbf{80}'80,'\textbf{85}'85,'\textbf{90}'90,'\textbf{95}'95,'\textbf{100}'100)
set ylabel '\large\textbf{Accuracy}' offset 3.0
set xlabel '\large\textbf{Class labels}'
set yrange [ 80: 100 ]
x = 0.0
## Last datafile plotted: "silver.dat"
plot 'silver.dat' using (1):2 lc rgb "magenta" title "Still",'silver.dat' using (2):3 lc rgb "green"title "Walk", 'silver.dat' using (3):4 lc rgb "blue" title "Run", 'silver.dat' using (4):5 lc rgb "red" title "Bike"


==> class_wise/m1/dbm/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3600.00,2520.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(946,1103){\makebox(0,0)[r]{\strut{}\textbf{85}}}%
      \csname LTb\endcsname%%
      \put(946,1502){\makebox(0,0)[r]{\strut{}\textbf{90}}}%
      \csname LTb\endcsname%%
      \put(946,1901){\makebox(0,0)[r]{\strut{}\textbf{95}}}%
      \csname LTb\endcsname%%
      \put(946,2300){\makebox(0,0)[r]{\strut{}\textbf{100}}}%
      \csname LTb\endcsname%%
      \put(1382,484){\makebox(0,0){\strut{}\large$\mathbf{f_1}$}}%
      \csname LTb\endcsname%%
      \put(1888,484){\makebox(0,0){\strut{}\large$\mathbf{f_2}$}}%
      \csname LTb\endcsname%%
      \put(2393,484){\makebox(0,0){\strut{}\large$\mathbf{f_3}$}}%
      \csname LTb\endcsname%%
      \put(2899,484){\makebox(0,0){\strut{}\large$\mathbf{f_4}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(594,1502){\rotatebox{-270}{\makebox(0,0){\strut{}\large\textbf{Accuracy}}}}%
      \put(2140,154){\makebox(0,0){\strut{}\large\textbf{Class labels}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> class_wise/m1/vbd/1 <==
set terminal epslatex;
set output '1.tex';
set size 0.5,0.5;
#set border 2 front lt black linewidth 1.000 dashtype solid
set boxwidth 0.4 absolute
set style fill solid 0.50 border lt -1
#set key horizontal
set grid
set key off
set pointsize 0.5
set style data boxplot
#set xtics border in scale 0,0  rotate  
#set xtics  offset -1,-1.5 norangelimit 
set xtics ('\large$\mathbf{g_1}$' 1, '\large$\mathbf{g_2}$' 2, '\large$\mathbf{g_3}$' 3, '\large$\mathbf{g_4}$' 4, '\large$\mathbf{g_5}$' 5)
set ytics ('\textbf{80}'80,'\textbf{85}'85,'\textbf{90}'90,'\textbf{95}'95,'\textbf{100}'100)
set ylabel '\large\textbf{Accuracy}' offset 3.0
set xlabel '\large\textbf{Class labels}'
set yrange [ 80: 100 ]
x = 0.0
## Last datafile plotted: "silver.dat"
plot 'silver.dat' using (1):2 lc rgb "magenta" title "Still",'silver.dat' using (2):3 lc rgb "green"title "Walk", 'silver.dat' using (3):4 lc rgb "blue" title "Run", 'silver.dat' using (4):5 lc rgb "red" title "Bike",'silver.dat' using (5):6 lc rgb "black" title "Bike"


==> class_wise/m1/vbd/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3600.00,2520.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(946,1103){\makebox(0,0)[r]{\strut{}\textbf{85}}}%
      \csname LTb\endcsname%%
      \put(946,1502){\makebox(0,0)[r]{\strut{}\textbf{90}}}%
      \csname LTb\endcsname%%
      \put(946,1901){\makebox(0,0)[r]{\strut{}\textbf{95}}}%
      \csname LTb\endcsname%%
      \put(946,2300){\makebox(0,0)[r]{\strut{}\textbf{100}}}%
      \csname LTb\endcsname%%
      \put(1323,484){\makebox(0,0){\strut{}\large$\mathbf{g_1}$}}%
      \csname LTb\endcsname%%
      \put(1732,484){\makebox(0,0){\strut{}\large$\mathbf{g_2}$}}%
      \csname LTb\endcsname%%
      \put(2141,484){\makebox(0,0){\strut{}\large$\mathbf{g_3}$}}%
      \csname LTb\endcsname%%
      \put(2549,484){\makebox(0,0){\strut{}\large$\mathbf{g_4}$}}%
      \csname LTb\endcsname%%
      \put(2958,484){\makebox(0,0){\strut{}\large$\mathbf{g_5}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(594,1502){\rotatebox{-270}{\makebox(0,0){\strut{}\large\textbf{Accuracy}}}}%
      \put(2140,154){\makebox(0,0){\strut{}\large\textbf{Class labels}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> class_wise/m2/1_ <==
set terminal epslatex;
set output '1.tex'; 
set size .73,.5;
set xlabel '{\footnotesize Regularization Parameter \alpha}';
set ylabel '{\footnotesize Overall Accuracy of Symbols}' offset 3;
set pointsize 1;
set ytics 0.65,0.1,1.0
set xtics ('$10^{-3}' 1, '$10^{-2}' 2, '$10^{-1}' 3, '$10^{0}' 4, '$10^{1}' 5)
plot [][0.55:0.95] 'res2.txt' using 1:2 with linespoints lt 1 lc rgb "red" lw 1 pt 1 title '\footnotesize No hidden layer','res2.txt' using 1:3 with linespoints lt 2 lc rgb "blue" lw 1 pt 2 title '\footnotesize One hidden layer','res2.txt' using 1:4 with linespoints lt 3 lc rgb "black" lw 1 pt 3 title '\footnotesize Two hidden layers'


==> class_wise/m2/dbd/1 <==
set terminal epslatex;
set output '1.tex';
set size 0.5,0.5;
#set border 2 front lt black linewidth 1.000 dashtype solid
set boxwidth 0.4 absolute
set style fill solid 0.50 border lt -1
#set key horizontal
set grid
set key off
set pointsize 0.5
set style data boxplot
#set xtics border in scale 0,0  rotate  
#set xtics  offset -1,-1.5 norangelimit 
set xtics ('\large$\mathbf{h_1}$' 1, '\large$\mathbf{h_2}$' 2, '\large$\mathbf{h_3}$' 3, '\large$\mathbf{h_4}$' 4)
set ytics ('\textbf{75}'75,'\textbf{80}'80,'\textbf{85}'85,'\textbf{90}'90,'\textbf{95}'95)
set ylabel '\large\textbf{Accuracy}' offset 2.0
set xlabel '\large\textbf{Class labels}'
set yrange [ 75: 95 ]
x = 0.0
## Last datafile plotted: "silver.dat"
plot 'silver.dat' using (1):2 lc rgb "magenta" title "Still",'silver.dat' using (2):3 lc rgb "green"title "Walk", 'silver.dat' using (3):4 lc rgb "blue" title "Run", 'silver.dat' using (4):5 lc rgb "red" title "Bike"


==> class_wise/m2/dbd/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3600.00,2520.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}\textbf{75}}}%
      \csname LTb\endcsname%%
      \put(814,1103){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(814,1502){\makebox(0,0)[r]{\strut{}\textbf{85}}}%
      \csname LTb\endcsname%%
      \put(814,1901){\makebox(0,0)[r]{\strut{}\textbf{90}}}%
      \csname LTb\endcsname%%
      \put(814,2300){\makebox(0,0)[r]{\strut{}\textbf{95}}}%
      \csname LTb\endcsname%%
      \put(1268,484){\makebox(0,0){\strut{}\large$\mathbf{h_1}$}}%
      \csname LTb\endcsname%%
      \put(1806,484){\makebox(0,0){\strut{}\large$\mathbf{h_2}$}}%
      \csname LTb\endcsname%%
      \put(2343,484){\makebox(0,0){\strut{}\large$\mathbf{h_3}$}}%
      \csname LTb\endcsname%%
      \put(2881,484){\makebox(0,0){\strut{}\large$\mathbf{h_4}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,1502){\rotatebox{-270}{\makebox(0,0){\strut{}\large\textbf{Accuracy}}}}%
      \put(2074,154){\makebox(0,0){\strut{}\large\textbf{Class labels}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> class_wise/m2/dbm/1 <==
set terminal epslatex;
set output '1.tex';
set size 0.5,0.5;
#set border 2 front lt black linewidth 1.000 dashtype solid
set boxwidth 0.4 absolute
set style fill solid 0.50 border lt -1
#set key horizontal
set grid
set key off
set pointsize 0.5
set style data boxplot
#set xtics border in scale 0,0  rotate  
#set xtics  offset -1,-1.5 norangelimit 
set xtics ('\large$\mathbf{f_1}$' 1, '\large$\mathbf{f_2}$' 2, '\large$\mathbf{f_3}$' 3, '\large$\mathbf{f_4}$' 4)
set ytics ('\textbf{75}' 75,'\textbf{80}'80,'\textbf{85}'85,'\textbf{90}'90,'\textbf{95}'95)
set ylabel '\large\textbf{Accuracy}' offset 2.0
set xlabel '\large\textbf{Class labels}'
set yrange [ 75: 95 ]
x = 0.0
## Last datafile plotted: "silver.dat"
plot 'silver.dat' using (1):2 lc rgb "magenta" title "Still",'silver.dat' using (2):3 lc rgb "green"title "Walk", 'silver.dat' using (3):4 lc rgb "blue" title "Run", 'silver.dat' using (4):5 lc rgb "red" title "Bike"


==> class_wise/m2/dbm/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3600.00,2520.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}\textbf{75}}}%
      \csname LTb\endcsname%%
      \put(814,1103){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(814,1502){\makebox(0,0)[r]{\strut{}\textbf{85}}}%
      \csname LTb\endcsname%%
      \put(814,1901){\makebox(0,0)[r]{\strut{}\textbf{90}}}%
      \csname LTb\endcsname%%
      \put(814,2300){\makebox(0,0)[r]{\strut{}\textbf{95}}}%
      \csname LTb\endcsname%%
      \put(1268,484){\makebox(0,0){\strut{}\large$\mathbf{f_1}$}}%
      \csname LTb\endcsname%%
      \put(1806,484){\makebox(0,0){\strut{}\large$\mathbf{f_2}$}}%
      \csname LTb\endcsname%%
      \put(2343,484){\makebox(0,0){\strut{}\large$\mathbf{f_3}$}}%
      \csname LTb\endcsname%%
      \put(2881,484){\makebox(0,0){\strut{}\large$\mathbf{f_4}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,1502){\rotatebox{-270}{\makebox(0,0){\strut{}\large\textbf{Accuracy}}}}%
      \put(2074,154){\makebox(0,0){\strut{}\large\textbf{Class labels}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> class_wise/m2/vbd/1 <==
set terminal epslatex;
set output '1.tex';
set size 0.5,0.5;
#set border 2 front lt black linewidth 1.000 dashtype solid
set boxwidth 0.4 absolute
set style fill solid 0.50 border lt -1
#set key horizontal
set grid
set key off
set pointsize 0.5
set style data boxplot
#set xtics border in scale 0,0  rotate  
#set xtics  offset -1,-1.5 norangelimit 
set xtics ('\large$\mathbf{g_1}$' 1, '\large$\mathbf{g_2}$' 2, '\large$\mathbf{g_3}$' 3, '\large$\mathbf{g_4}$' 4, '\large$\mathbf{g_5}$' 5)
set ytics ('\textbf{75}'75,'\textbf{80}'80,'\textbf{85}'85,'\textbf{90}'90,'\textbf{95}'95)
set ylabel '\large\textbf{Accuracy}' offset 2.0
set xlabel '\large\textbf{Class labels}'
set yrange [ 75: 95 ]
x = 0.0
## Last datafile plotted: "silver.dat"
plot 'silver.dat' using (1):2 lc rgb "magenta" title "Still",'silver.dat' using (2):3 lc rgb "green"title "Walk", 'silver.dat' using (3):4 lc rgb "blue" title "Run", 'silver.dat' using (4):5 lc rgb "red" title "Bike",'silver.dat' using (5):6 lc rgb "black" title "Bike"


==> class_wise/m2/vbd/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3600.00,2520.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}\textbf{75}}}%
      \csname LTb\endcsname%%
      \put(814,1103){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(814,1502){\makebox(0,0)[r]{\strut{}\textbf{85}}}%
      \csname LTb\endcsname%%
      \put(814,1901){\makebox(0,0)[r]{\strut{}\textbf{90}}}%
      \csname LTb\endcsname%%
      \put(814,2300){\makebox(0,0)[r]{\strut{}\textbf{95}}}%
      \csname LTb\endcsname%%
      \put(1206,484){\makebox(0,0){\strut{}\large$\mathbf{g_1}$}}%
      \csname LTb\endcsname%%
      \put(1640,484){\makebox(0,0){\strut{}\large$\mathbf{g_2}$}}%
      \csname LTb\endcsname%%
      \put(2075,484){\makebox(0,0){\strut{}\large$\mathbf{g_3}$}}%
      \csname LTb\endcsname%%
      \put(2509,484){\makebox(0,0){\strut{}\large$\mathbf{g_4}$}}%
      \csname LTb\endcsname%%
      \put(2943,484){\makebox(0,0){\strut{}\large$\mathbf{g_5}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,1502){\rotatebox{-270}{\makebox(0,0){\strut{}\large\textbf{Accuracy}}}}%
      \put(2074,154){\makebox(0,0){\strut{}\large\textbf{Class labels}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> conf_mat_dbd/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> conf_mat_dbm/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> conf_mat_vdb/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> epoch_accuracy/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> epoch_accuracy/DBD/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.6;
#set pointsize 1.5;
set xlabel '\large{\textbf{Epoch}}' offset 1;
set ylabel '\large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 2;
#set ytics 60,5,100
set xtics 10,10,100 
set grid
set key right bottom Right 
set xtics ("20" 20, "40" 40,"60" 60, "80" 80, "100" 100, "120" 120,"140" 140,"160" 160,"180" 180,"200" 200);
set ytics ("55"55,"60" 60, "65" 65,"70" 70, "75" 75, "80" 80,"85" 85, "90" 90,"95" 95,"100" 100);

#set object 1 ellipse center 100,97.5 size 8.5, 4.8 angle 0 front fc rgb"olive" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Negligible change' at 96,93.5;


plot [8:208][55:100] 'final_out_d1' using 1:2 with linespoints lt 4 lc rgb "red" lw 5 title '\large $\mathbf{M}^t$', 'final_out_d1' using 1:3 with linespoints lt 2 lc rgb "blue" lw 5 title '\large $\mathbf{M}^s_1$','final_out_d1' using 1:4 with linespoints lt 3 lc rgb "dark-green" lw 5 title '\large $\mathbf{M}^s_2$'


==> epoch_accuracy/DBD/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}55}}%
      \csname LTb\endcsname%%
      \put(814,937){\makebox(0,0)[r]{\strut{}60}}%
      \csname LTb\endcsname%%
      \put(814,1170){\makebox(0,0)[r]{\strut{}65}}%
      \csname LTb\endcsname%%
      \put(814,1404){\makebox(0,0)[r]{\strut{}70}}%
      \csname LTb\endcsname%%
      \put(814,1637){\makebox(0,0)[r]{\strut{}75}}%
      \csname LTb\endcsname%%
      \put(814,1870){\makebox(0,0)[r]{\strut{}80}}%
      \csname LTb\endcsname%%
      \put(814,2103){\makebox(0,0)[r]{\strut{}85}}%
      \csname LTb\endcsname%%
      \put(814,2337){\makebox(0,0)[r]{\strut{}90}}%
      \csname LTb\endcsname%%
      \put(814,2570){\makebox(0,0)[r]{\strut{}95}}%
      \csname LTb\endcsname%%
      \put(814,2803){\makebox(0,0)[r]{\strut{}100}}%
      \csname LTb\endcsname%%
      \put(1168,484){\makebox(0,0){\strut{}20}}%
      \csname LTb\endcsname%%
      \put(1538,484){\makebox(0,0){\strut{}40}}%
      \csname LTb\endcsname%%
      \put(1907,484){\makebox(0,0){\strut{}60}}%
      \csname LTb\endcsname%%
      \put(2277,484){\makebox(0,0){\strut{}80}}%
      \csname LTb\endcsname%%
      \put(2647,484){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(3016,484){\makebox(0,0){\strut{}120}}%
      \csname LTb\endcsname%%
      \put(3386,484){\makebox(0,0){\strut{}140}}%
      \csname LTb\endcsname%%
      \put(3756,484){\makebox(0,0){\strut{}160}}%
      \csname LTb\endcsname%%
      \put(4125,484){\makebox(0,0){\strut{}180}}%
      \csname LTb\endcsname%%
      \put(4495,484){\makebox(0,0){\strut{}200}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(330,1753){\rotatebox{-270}{\makebox(0,0){\strut{}\large{\textbf{Accuracy (\%)}}}}}%
      \put(2926,154){\makebox(0,0){\strut{}\large{\textbf{Epoch}}}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^t$}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_1$}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_accuracy/DBD/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_accuracy/DBM/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.6;
#set pointsize 1.5;
set xlabel '\large{\textbf{Epoch}}' offset 1;
set ylabel '\large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 2;
#set ytics 60,5,100
set xtics 10,10,100 
set grid
set key right bottom Right 
set xtics ("20" 20, "40" 40,"60" 60, "80" 80, "100" 100, "120" 120,"140" 140,"160" 160,"180" 180,"200" 200);
set ytics ("60" 60, "65" 65,"70" 70, "75" 75, "80" 80,"85" 85, "90" 90,"95" 95,"100" 100);

#set object 1 ellipse center 100,97.5 size 8.5, 4.8 angle 0 front fc rgb"olive" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Negligible change' at 96,93.5;


plot [8:208][60:100] 'final_out_d1' using 1:2 with linespoints lt 4 lc rgb "red" lw 5 title '\large $\mathbf{M}^t$', 'final_out_d1' using 1:3 with linespoints lt 2 lc rgb "blue" lw 5 title '\large $\mathbf{M}^s_1$','final_out_d1' using 1:4 with linespoints lt 3 lc rgb "dark-green" lw 5 title '\large $\mathbf{M}^s_2$'


==> epoch_accuracy/DBM/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}60}}%
      \csname LTb\endcsname%%
      \put(814,966){\makebox(0,0)[r]{\strut{}65}}%
      \csname LTb\endcsname%%
      \put(814,1229){\makebox(0,0)[r]{\strut{}70}}%
      \csname LTb\endcsname%%
      \put(814,1491){\makebox(0,0)[r]{\strut{}75}}%
      \csname LTb\endcsname%%
      \put(814,1754){\makebox(0,0)[r]{\strut{}80}}%
      \csname LTb\endcsname%%
      \put(814,2016){\makebox(0,0)[r]{\strut{}85}}%
      \csname LTb\endcsname%%
      \put(814,2278){\makebox(0,0)[r]{\strut{}90}}%
      \csname LTb\endcsname%%
      \put(814,2541){\makebox(0,0)[r]{\strut{}95}}%
      \csname LTb\endcsname%%
      \put(814,2803){\makebox(0,0)[r]{\strut{}100}}%
      \csname LTb\endcsname%%
      \put(1168,484){\makebox(0,0){\strut{}20}}%
      \csname LTb\endcsname%%
      \put(1538,484){\makebox(0,0){\strut{}40}}%
      \csname LTb\endcsname%%
      \put(1907,484){\makebox(0,0){\strut{}60}}%
      \csname LTb\endcsname%%
      \put(2277,484){\makebox(0,0){\strut{}80}}%
      \csname LTb\endcsname%%
      \put(2647,484){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(3016,484){\makebox(0,0){\strut{}120}}%
      \csname LTb\endcsname%%
      \put(3386,484){\makebox(0,0){\strut{}140}}%
      \csname LTb\endcsname%%
      \put(3756,484){\makebox(0,0){\strut{}160}}%
      \csname LTb\endcsname%%
      \put(4125,484){\makebox(0,0){\strut{}180}}%
      \csname LTb\endcsname%%
      \put(4495,484){\makebox(0,0){\strut{}200}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(330,1753){\rotatebox{-270}{\makebox(0,0){\strut{}\large{\textbf{Accuracy (\%)}}}}}%
      \put(2926,154){\makebox(0,0){\strut{}\large{\textbf{Epoch}}}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^t$}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_1$}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_accuracy/DBM/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_accuracy/VDB/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.6;
#set pointsize 1.5;
set xlabel '\large{\textbf{Epoch}}' offset 1;
set ylabel '\large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 2;
#set ytics 60,5,100
set xtics 10,10,100 
set grid
set key right bottom Right 
set xtics ("20" 20, "40" 40,"60" 60, "80" 80, "100" 100, "120" 120,"140" 140,"160" 160,"180" 180,"200" 200);
set ytics ("60" 60, "65" 65,"70" 70, "75" 75, "80" 80,"85" 85, "90" 90,"95" 95,"100" 100);

#set object 1 ellipse center 100,97.5 size 8.5, 4.8 angle 0 front fc rgb"olive" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Negligible change' at 96,93.5;


plot [8:208][60:100] 'final_out_d1' using 1:2 with linespoints lt 4 lc rgb "red" lw 5 title '\large $\mathbf{M}^t$', 'final_out_d1' using 1:3 with linespoints lt 2 lc rgb "blue" lw 5 title '\large $\mathbf{M}^s_1$','final_out_d1' using 1:4 with linespoints lt 3 lc rgb "dark-green" lw 5 title '\large $\mathbf{M}^s_2$'


==> epoch_accuracy/VDB/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}60}}%
      \csname LTb\endcsname%%
      \put(814,966){\makebox(0,0)[r]{\strut{}65}}%
      \csname LTb\endcsname%%
      \put(814,1229){\makebox(0,0)[r]{\strut{}70}}%
      \csname LTb\endcsname%%
      \put(814,1491){\makebox(0,0)[r]{\strut{}75}}%
      \csname LTb\endcsname%%
      \put(814,1754){\makebox(0,0)[r]{\strut{}80}}%
      \csname LTb\endcsname%%
      \put(814,2016){\makebox(0,0)[r]{\strut{}85}}%
      \csname LTb\endcsname%%
      \put(814,2278){\makebox(0,0)[r]{\strut{}90}}%
      \csname LTb\endcsname%%
      \put(814,2541){\makebox(0,0)[r]{\strut{}95}}%
      \csname LTb\endcsname%%
      \put(814,2803){\makebox(0,0)[r]{\strut{}100}}%
      \csname LTb\endcsname%%
      \put(1168,484){\makebox(0,0){\strut{}20}}%
      \csname LTb\endcsname%%
      \put(1538,484){\makebox(0,0){\strut{}40}}%
      \csname LTb\endcsname%%
      \put(1907,484){\makebox(0,0){\strut{}60}}%
      \csname LTb\endcsname%%
      \put(2277,484){\makebox(0,0){\strut{}80}}%
      \csname LTb\endcsname%%
      \put(2647,484){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(3016,484){\makebox(0,0){\strut{}120}}%
      \csname LTb\endcsname%%
      \put(3386,484){\makebox(0,0){\strut{}140}}%
      \csname LTb\endcsname%%
      \put(3756,484){\makebox(0,0){\strut{}160}}%
      \csname LTb\endcsname%%
      \put(4125,484){\makebox(0,0){\strut{}180}}%
      \csname LTb\endcsname%%
      \put(4495,484){\makebox(0,0){\strut{}200}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(330,1753){\rotatebox{-270}{\makebox(0,0){\strut{}\large{\textbf{Accuracy (\%)}}}}}%
      \put(2926,154){\makebox(0,0){\strut{}\large{\textbf{Epoch}}}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^t$}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_1$}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_accuracy/VDB/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_fmeasure/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> epoch_fmeasure/DBD/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.6;
#set pointsize 1.5;
set xlabel '\large{\textbf{Epoch}}' offset 1;
set ylabel '\large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 2;
#set ytics 60,5,100
set xtics 10,10,100 
set grid
set key right bottom Right 
set xtics ("20" 20, "40" 40,"60" 60, "80" 80, "100" 100, "120" 120,"140" 140,"160" 160,"180" 180,"200" 200);
set ytics ("55"55,"60" 60, "65" 65,"70" 70, "75" 75, "80" 80,"85" 85, "90" 90,"95" 95,"100" 100);

#set object 1 ellipse center 100,97.5 size 8.5, 4.8 angle 0 front fc rgb"olive" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Negligible change' at 96,93.5;


plot [8:208][55:100] 'final_out_d1' using 1:2 with linespoints lt 4 lc rgb "red" lw 5 title '\large $\mathbf{M}^t$', 'final_out_d1' using 1:3 with linespoints lt 2 lc rgb "blue" lw 5 title '\large $\mathbf{M}^s_1$','final_out_d1' using 1:4 with linespoints lt 3 lc rgb "dark-green" lw 5 title '\large $\mathbf{M}^s_2$'


==> epoch_fmeasure/DBD/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}55}}%
      \csname LTb\endcsname%%
      \put(814,937){\makebox(0,0)[r]{\strut{}60}}%
      \csname LTb\endcsname%%
      \put(814,1170){\makebox(0,0)[r]{\strut{}65}}%
      \csname LTb\endcsname%%
      \put(814,1404){\makebox(0,0)[r]{\strut{}70}}%
      \csname LTb\endcsname%%
      \put(814,1637){\makebox(0,0)[r]{\strut{}75}}%
      \csname LTb\endcsname%%
      \put(814,1870){\makebox(0,0)[r]{\strut{}80}}%
      \csname LTb\endcsname%%
      \put(814,2103){\makebox(0,0)[r]{\strut{}85}}%
      \csname LTb\endcsname%%
      \put(814,2337){\makebox(0,0)[r]{\strut{}90}}%
      \csname LTb\endcsname%%
      \put(814,2570){\makebox(0,0)[r]{\strut{}95}}%
      \csname LTb\endcsname%%
      \put(814,2803){\makebox(0,0)[r]{\strut{}100}}%
      \csname LTb\endcsname%%
      \put(1168,484){\makebox(0,0){\strut{}20}}%
      \csname LTb\endcsname%%
      \put(1538,484){\makebox(0,0){\strut{}40}}%
      \csname LTb\endcsname%%
      \put(1907,484){\makebox(0,0){\strut{}60}}%
      \csname LTb\endcsname%%
      \put(2277,484){\makebox(0,0){\strut{}80}}%
      \csname LTb\endcsname%%
      \put(2647,484){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(3016,484){\makebox(0,0){\strut{}120}}%
      \csname LTb\endcsname%%
      \put(3386,484){\makebox(0,0){\strut{}140}}%
      \csname LTb\endcsname%%
      \put(3756,484){\makebox(0,0){\strut{}160}}%
      \csname LTb\endcsname%%
      \put(4125,484){\makebox(0,0){\strut{}180}}%
      \csname LTb\endcsname%%
      \put(4495,484){\makebox(0,0){\strut{}200}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(330,1753){\rotatebox{-270}{\makebox(0,0){\strut{}\large{\textbf{Accuracy (\%)}}}}}%
      \put(2926,154){\makebox(0,0){\strut{}\large{\textbf{Epoch}}}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^t$}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_1$}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_fmeasure/DBD/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_fmeasure/DBM/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.6;
#set pointsize 1.5;
set xlabel '\large{\textbf{Epoch}}' offset 1;
set ylabel '\large{\textbf{F$_1$ score (\%)}}' offset 1;
set pointsize 2;
#set ytics 60,5,100
set xtics 10,10,100 
set grid
set key right bottom Right 
set xtics ("20" 20, "40" 40,"60" 60, "80" 80, "100" 100, "120" 120,"140" 140,"160" 160,"180" 180,"200" 200);
set ytics ("60" 60, "65" 65,"70" 70, "75" 75, "80" 80,"85" 85, "90" 90,"95" 95,"100" 100);

#set object 1 ellipse center 100,97.5 size 8.5, 4.8 angle 0 front fc rgb"olive" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Negligible change' at 96,93.5;


plot [8:208][60:100] 'final_out_d1' using 1:2 with linespoints lt 4 lc rgb "red" lw 5 title '\large $\mathbf{M}^t$', 'final_out_d1' using 1:3 with linespoints lt 2 lc rgb "blue" lw 5 title '\large $\mathbf{M}^s_1$','final_out_d1' using 1:4 with linespoints lt 3 lc rgb "dark-green" lw 5 title '\large $\mathbf{M}^s_2$'


==> epoch_fmeasure/DBM/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}60}}%
      \csname LTb\endcsname%%
      \put(814,966){\makebox(0,0)[r]{\strut{}65}}%
      \csname LTb\endcsname%%
      \put(814,1229){\makebox(0,0)[r]{\strut{}70}}%
      \csname LTb\endcsname%%
      \put(814,1491){\makebox(0,0)[r]{\strut{}75}}%
      \csname LTb\endcsname%%
      \put(814,1754){\makebox(0,0)[r]{\strut{}80}}%
      \csname LTb\endcsname%%
      \put(814,2016){\makebox(0,0)[r]{\strut{}85}}%
      \csname LTb\endcsname%%
      \put(814,2278){\makebox(0,0)[r]{\strut{}90}}%
      \csname LTb\endcsname%%
      \put(814,2541){\makebox(0,0)[r]{\strut{}95}}%
      \csname LTb\endcsname%%
      \put(814,2803){\makebox(0,0)[r]{\strut{}100}}%
      \csname LTb\endcsname%%
      \put(1168,484){\makebox(0,0){\strut{}20}}%
      \csname LTb\endcsname%%
      \put(1538,484){\makebox(0,0){\strut{}40}}%
      \csname LTb\endcsname%%
      \put(1907,484){\makebox(0,0){\strut{}60}}%
      \csname LTb\endcsname%%
      \put(2277,484){\makebox(0,0){\strut{}80}}%
      \csname LTb\endcsname%%
      \put(2647,484){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(3016,484){\makebox(0,0){\strut{}120}}%
      \csname LTb\endcsname%%
      \put(3386,484){\makebox(0,0){\strut{}140}}%
      \csname LTb\endcsname%%
      \put(3756,484){\makebox(0,0){\strut{}160}}%
      \csname LTb\endcsname%%
      \put(4125,484){\makebox(0,0){\strut{}180}}%
      \csname LTb\endcsname%%
      \put(4495,484){\makebox(0,0){\strut{}200}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(330,1753){\rotatebox{-270}{\makebox(0,0){\strut{}\large{\textbf{F$_1$ score (\%)}}}}}%
      \put(2926,154){\makebox(0,0){\strut{}\large{\textbf{Epoch}}}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^t$}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_1$}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_fmeasure/DBM/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_fmeasure/VDB/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.6;
#set pointsize 1.5;
set xlabel '\large{\textbf{Epoch}}' offset 1;
set ylabel '\large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 2;
#set ytics 60,5,100
set xtics 10,10,100 
set grid
set key right bottom Right 
set xtics ("20" 20, "40" 40,"60" 60, "80" 80, "100" 100, "120" 120,"140" 140,"160" 160,"180" 180,"200" 200);
set ytics ("55"55,"60" 60, "65" 65,"70" 70, "75" 75, "80" 80,"85" 85, "90" 90,"95" 95,"100" 100);

#set object 1 ellipse center 100,97.5 size 8.5, 4.8 angle 0 front fc rgb"olive" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Negligible change' at 96,93.5;


plot [8:208][55:100] 'final_out_d1' using 1:2 with linespoints lt 4 lc rgb "red" lw 5 title '\large $\mathbf{M}^t$', 'final_out_d1' using 1:3 with linespoints lt 2 lc rgb "blue" lw 5 title '\large $\mathbf{M}^s_1$','final_out_d1' using 1:4 with linespoints lt 3 lc rgb "dark-green" lw 5 title '\large $\mathbf{M}^s_2$'


==> epoch_fmeasure/VDB/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}55}}%
      \csname LTb\endcsname%%
      \put(814,937){\makebox(0,0)[r]{\strut{}60}}%
      \csname LTb\endcsname%%
      \put(814,1170){\makebox(0,0)[r]{\strut{}65}}%
      \csname LTb\endcsname%%
      \put(814,1404){\makebox(0,0)[r]{\strut{}70}}%
      \csname LTb\endcsname%%
      \put(814,1637){\makebox(0,0)[r]{\strut{}75}}%
      \csname LTb\endcsname%%
      \put(814,1870){\makebox(0,0)[r]{\strut{}80}}%
      \csname LTb\endcsname%%
      \put(814,2103){\makebox(0,0)[r]{\strut{}85}}%
      \csname LTb\endcsname%%
      \put(814,2337){\makebox(0,0)[r]{\strut{}90}}%
      \csname LTb\endcsname%%
      \put(814,2570){\makebox(0,0)[r]{\strut{}95}}%
      \csname LTb\endcsname%%
      \put(814,2803){\makebox(0,0)[r]{\strut{}100}}%
      \csname LTb\endcsname%%
      \put(1168,484){\makebox(0,0){\strut{}20}}%
      \csname LTb\endcsname%%
      \put(1538,484){\makebox(0,0){\strut{}40}}%
      \csname LTb\endcsname%%
      \put(1907,484){\makebox(0,0){\strut{}60}}%
      \csname LTb\endcsname%%
      \put(2277,484){\makebox(0,0){\strut{}80}}%
      \csname LTb\endcsname%%
      \put(2647,484){\makebox(0,0){\strut{}100}}%
      \csname LTb\endcsname%%
      \put(3016,484){\makebox(0,0){\strut{}120}}%
      \csname LTb\endcsname%%
      \put(3386,484){\makebox(0,0){\strut{}140}}%
      \csname LTb\endcsname%%
      \put(3756,484){\makebox(0,0){\strut{}160}}%
      \csname LTb\endcsname%%
      \put(4125,484){\makebox(0,0){\strut{}180}}%
      \csname LTb\endcsname%%
      \put(4495,484){\makebox(0,0){\strut{}200}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(330,1753){\rotatebox{-270}{\makebox(0,0){\strut{}\large{\textbf{Accuracy (\%)}}}}}%
      \put(2926,154){\makebox(0,0){\strut{}\large{\textbf{Epoch}}}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^t$}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_1$}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> epoch_fmeasure/VDB/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> execution/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 1.10,0.6;
set ylabel '\small Compression (in \%)' offset 2;
set xlabel '\small Approaches' offset 0;
set xtics ('\hspace{0.2cm}\small ADONN' 0.8, '\hspace{0.2cm} \small DLFDB' 1.6, '\hspace{0.2cm} \small SenseHAR' 2.4,'\hspace{0.2cm} \small \textcolor{red}{Proposed}' 3.2 )
#set xtic rotate by -45 scale 0
set ytics ('\scriptsize 10' 10, '\scriptsize 20' 20, '\scriptsize 30' 30, '\scriptsize 40' 40, '\scriptsize 50' 50) 
set grid
#set key horizontal maxrow 1 samplen 1 
#set key horizontal
set key at 2.50,53 horizontal 
#maxrow 1 samplen 0.8
#set key at 4.3, 0.57 width -3.75 opaque box maxrow 1.5 
set boxwidth 0.20 relative
set style fill solid 0.9
plot [0.3:3.7][0:55] "final_out_d1" u ($1-0.10):2 w boxes fill pattern 9 lc rgb "#21908d" lw 4 title '\large $\mathbf{M}^s_1$', "final_out_d1" u ($1+0.10):3 w boxes fill pattern 2 lc rgb "#8B0000" lw 3 title '\large $\mathbf{M}^s_2$'


==> execution/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7920.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,1086){\makebox(0,0)[r]{\strut{}\scriptsize 10}}%
      \csname LTb\endcsname%%
      \put(946,1467){\makebox(0,0)[r]{\strut{}\scriptsize 20}}%
      \csname LTb\endcsname%%
      \put(946,1849){\makebox(0,0)[r]{\strut{}\scriptsize 30}}%
      \csname LTb\endcsname%%
      \put(946,2231){\makebox(0,0)[r]{\strut{}\scriptsize 40}}%
      \csname LTb\endcsname%%
      \put(946,2612){\makebox(0,0)[r]{\strut{}\scriptsize 50}}%
      \csname LTb\endcsname%%
      \put(2026,484){\makebox(0,0){\strut{}\hspace{0.2cm}\small ADONN}}%
      \csname LTb\endcsname%%
      \put(3542,484){\makebox(0,0){\strut{}\hspace{0.2cm} \small DLFDB}}%
      \csname LTb\endcsname%%
      \put(5058,484){\makebox(0,0){\strut{}\hspace{0.2cm} \small SenseHAR}}%
      \csname LTb\endcsname%%
      \put(6574,484){\makebox(0,0){\strut{}\hspace{0.2cm} \small \textcolor{red}{Proposed}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,1753){\rotatebox{-270}{\makebox(0,0){\strut{}\small Compression (in \%)}}}%
      \put(4300,154){\makebox(0,0){\strut{}\small Approaches}}%
      \csname LTb\endcsname%%
      \put(2746,2617){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_1$}}%
      \csname LTb\endcsname%%
      \put(4393,2617){\makebox(0,0)[r]{\strut{}\large $\mathbf{M}^s_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> execution/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> execution/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> execution1/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 1.3,0.6;
set ylabel '\small Execution time (in ms)' offset 4.0;
set xlabel '\small Devices' offset 0;
set xtics ('$\mathbf{d_1}$' 4, '$\mathbf{d_2}$' 8, '$\mathbf{d_3}$' 12,'$\mathbf{d_4}$' 16,'$\mathbf{d_5}$' 20 )
#set xtic rotate by -45 scale 0
set ytics ('\small 20' 20, '\small 50' 40, '\small 200' 60, '\small 1000' 80,'\small 5000' 100,'\small 20000' 120,'\small 80000' 140) 
set grid
set key horizontal maxrow 1 samplen 1 top
#set key horizontal
#set key at 2.50,53 horizontal 
#maxrow 1 samplen 0.8
#set key at 4.3, 0.57 width -3.75 opaque box maxrow 1.5 
set boxwidth 0.10 relative
set style fill solid 0.9
plot [2:22][0:140] "final_out_d1" u ($1-1.25):2 w boxes fill  lc rgb "#21908d" lw 4 title '\large DeepZero', "final_out_d1" u ($1-0.75):3 w boxes fill  lc rgb "#8B0000" lw 3 title '\large [2]',"final_out_d1" u ($1-0.25):4 w boxes fill  lc rgb "#006400" lw 3 title '\large DeepSense',"final_out_d1" u ($1+0.25):7 w boxes fill lc rgb "#800080" lw 3 title '\large DT-MIL',"final_out_d1" u ($1+0.75):6 w boxes fill  lc rgb "blue" lw 3 title '\large DeepFusion',"final_out_d1" u ($1+1.25):7 w boxes fill  lc rgb "red" lw 3 title '\large [6]'


==> execution1/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9360.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1342,1004){\makebox(0,0)[r]{\strut{}\small 20}}%
      \csname LTb\endcsname%%
      \put(1342,1304){\makebox(0,0)[r]{\strut{}\small 50}}%
      \csname LTb\endcsname%%
      \put(1342,1604){\makebox(0,0)[r]{\strut{}\small 200}}%
      \csname LTb\endcsname%%
      \put(1342,1903){\makebox(0,0)[r]{\strut{}\small 1000}}%
      \csname LTb\endcsname%%
      \put(1342,2203){\makebox(0,0)[r]{\strut{}\small 5000}}%
      \csname LTb\endcsname%%
      \put(1342,2503){\makebox(0,0)[r]{\strut{}\small 20000}}%
      \csname LTb\endcsname%%
      \put(1342,2803){\makebox(0,0)[r]{\strut{}\small 80000}}%
      \csname LTb\endcsname%%
      \put(2223,484){\makebox(0,0){\strut{}$\mathbf{d_1}$}}%
      \csname LTb\endcsname%%
      \put(3720,484){\makebox(0,0){\strut{}$\mathbf{d_2}$}}%
      \csname LTb\endcsname%%
      \put(5218,484){\makebox(0,0){\strut{}$\mathbf{d_3}$}}%
      \csname LTb\endcsname%%
      \put(6716,484){\makebox(0,0){\strut{}$\mathbf{d_4}$}}%
      \csname LTb\endcsname%%
      \put(8213,484){\makebox(0,0){\strut{}$\mathbf{d_5}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(726,1753){\rotatebox{-270}{\makebox(0,0){\strut{}\small Execution time (in ms)}}}%
      \put(5218,154){\makebox(0,0){\strut{}\small Devices}}%
      \csname LTb\endcsname%%
      \put(4285,2630){\makebox(0,0)[r]{\strut{}\large DeepZero}}%
      \csname LTb\endcsname%%
      \put(4285,2410){\makebox(0,0)[r]{\strut{}\large [2]}}%
      \csname LTb\endcsname%%
      \put(6328,2630){\makebox(0,0)[r]{\strut{}\large DeepSense}}%
      \csname LTb\endcsname%%
      \put(6328,2410){\makebox(0,0)[r]{\strut{}\large DT-MIL}}%
      \csname LTb\endcsname%%
      \put(8371,2630){\makebox(0,0)[r]{\strut{}\large DeepFusion}}%
      \csname LTb\endcsname%%
      \put(8371,2410){\makebox(0,0)[r]{\strut{}\large [6]}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> execution1/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> execution1/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> kd/m1/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.7,0.6;
set ylabel '\large Accuracy  ($\%$)' offset 2.0;
set xlabel '\large Dataset' offset 0;
set xtics ('\hspace{0.3cm}\textbf{DBM}' 1, '\hspace{0.3cm}\textbf{VDB}' 2, '\hspace{0.3cm}\textbf{DBD}' 3, '\hspace{0.3cm}\textbf{Avg.}' 4)
#set xtic rotate by -45 scale 0
set ytics ('\textbf{75}' 75, '\textbf{80}' 80, '\textbf{85}' 85, '\textbf{90}' 90, '\textbf{95}' 95) 
set grid
#set key top horizontal
set key at 4.25, 98.0 width -0.5 opaque box maxrow 1 
set key samplen 2
set key width -2.5 
set boxwidth 0.25 relative
set style fill solid 0.9
plot [0.5:4.5][70:99] "final_out_d1" u ($1-0.15):2 w boxes fill pattern 9 lc rgb "#8B0000" lw 4 title 'with KD', "final_out_d1" u ($1+0.15):3 w boxes fill pattern 2 lc rgb "#2E8B57" lw 3 title 'without KD'


==> kd/m1/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,1066){\makebox(0,0)[r]{\strut{}\textbf{75}}}%
      \csname LTb\endcsname%%
      \put(814,1428){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(814,1790){\makebox(0,0)[r]{\strut{}\textbf{85}}}%
      \csname LTb\endcsname%%
      \put(814,2152){\makebox(0,0)[r]{\strut{}\textbf{90}}}%
      \csname LTb\endcsname%%
      \put(814,2513){\makebox(0,0)[r]{\strut{}\textbf{95}}}%
      \csname LTb\endcsname%%
      \put(1408,484){\makebox(0,0){\strut{}\hspace{0.3cm}\textbf{DBM}}}%
      \csname LTb\endcsname%%
      \put(2332,484){\makebox(0,0){\strut{}\hspace{0.3cm}\textbf{VDB}}}%
      \csname LTb\endcsname%%
      \put(3257,484){\makebox(0,0){\strut{}\hspace{0.3cm}\textbf{DBD}}}%
      \csname LTb\endcsname%%
      \put(4181,484){\makebox(0,0){\strut{}\hspace{0.3cm}\textbf{Avg.}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,1753){\rotatebox{-270}{\makebox(0,0){\strut{}\large Accuracy  ($\%$)}}}%
      \put(2794,154){\makebox(0,0){\strut{}\large Dataset}}%
      \csname LTb\endcsname%%
      \put(2240,2621){\makebox(0,0)[r]{\strut{}with KD}}%
      \csname LTb\endcsname%%
      \put(3821,2621){\makebox(0,0)[r]{\strut{}without KD}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> kd/m1/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> kd/m1/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> kd/m2/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.7,0.6;
set ylabel '\large Accuracy  ($\%$)' offset 2.0;
set xlabel '\large Dataset' offset 0;
set xtics ('\hspace{0.3cm}\textbf{DBM}' 1, '\hspace{0.3cm}\textbf{VDB}' 2, '\hspace{0.3cm}\textbf{DBD}' 3, '\hspace{0.3cm}\textbf{Avg.}' 4)
#set xtic rotate by -45 scale 0
set ytics ( '\textbf{70}' 70,'\textbf{75}' 75, '\textbf{80}' 80, '\textbf{85}' 85, '\textbf{90}' 90) 
set grid
#set key top horizontal right
set key at 4.25, 93.0 width -0.5 opaque box maxrow 1 
set key samplen 2
set key width -2
set boxwidth 0.25 relative
set style fill solid 0.9
plot [0.5:4.5][65:94] "final_out_d1" u ($1-0.15):2 w boxes fill pattern 9 lc rgb "#8B0000" lw 4 title 'with KD', "final_out_d1" u ($1+0.15):3 w boxes fill pattern 2 lc rgb "#2E8B57" lw 3 title 'without KD'


==> kd/m2/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,1066){\makebox(0,0)[r]{\strut{}\textbf{70}}}%
      \csname LTb\endcsname%%
      \put(814,1428){\makebox(0,0)[r]{\strut{}\textbf{75}}}%
      \csname LTb\endcsname%%
      \put(814,1790){\makebox(0,0)[r]{\strut{}\textbf{80}}}%
      \csname LTb\endcsname%%
      \put(814,2152){\makebox(0,0)[r]{\strut{}\textbf{85}}}%
      \csname LTb\endcsname%%
      \put(814,2513){\makebox(0,0)[r]{\strut{}\textbf{90}}}%
      \csname LTb\endcsname%%
      \put(1408,484){\makebox(0,0){\strut{}\hspace{0.3cm}\textbf{DBM}}}%
      \csname LTb\endcsname%%
      \put(2332,484){\makebox(0,0){\strut{}\hspace{0.3cm}\textbf{VDB}}}%
      \csname LTb\endcsname%%
      \put(3257,484){\makebox(0,0){\strut{}\hspace{0.3cm}\textbf{DBD}}}%
      \csname LTb\endcsname%%
      \put(4181,484){\makebox(0,0){\strut{}\hspace{0.3cm}\textbf{Avg.}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,1753){\rotatebox{-270}{\makebox(0,0){\strut{}\large Accuracy  ($\%$)}}}%
      \put(2794,154){\makebox(0,0){\strut{}\large Dataset}}%
      \csname LTb\endcsname%%
      \put(2174,2621){\makebox(0,0)[r]{\strut{}with KD}}%
      \csname LTb\endcsname%%
      \put(3821,2621){\makebox(0,0)[r]{\strut{}without KD}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> kd/m2/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> kd/m2/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> proto1/flops/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> unseen_class_execution/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 1,0.6;
#set xlabel "Human Activities"
set ylabel '\large {\textbf{Performance} (\%)}' offset 1;
set xtics ('std\_talk' 1, 'sit\_sofa' 2, 'sit\_floor' 3, 'lyg\_bed' 4, 'lyg\_floor' 5, 'walk\_down' 6, 'walk\_up' 7, "eating" 8)
set xtic rotate by -45 scale 0
set ytics 0,20,100
#set grid
set key horizontal
set boxwidth 0.25 relative
set style fill solid 0.9
plot [0:9][0:120]"final_out_d" u 1:2 w boxes fill pattern 1 lc rgb"green" title 'Accuracy', "final_out_d" u ($1+0.3):3 w boxes fill pattern 2 lc rgb"blue" title 'Earliness'


==> unseen_class_memory/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 1,0.6;
#set xlabel "Human Activities"
set ylabel '\large {\textbf{Performance} (\%)}' offset 1;
set xtics ('std\_talk' 1, 'sit\_sofa' 2, 'sit\_floor' 3, 'lyg\_bed' 4, 'lyg\_floor' 5, 'walk\_down' 6, 'walk\_up' 7, "eating" 8)
set xtic rotate by -45 scale 0
set ytics 0,20,100
#set grid
set key horizontal
set boxwidth 0.25 relative
set style fill solid 0.9
plot [0:9][0:120]"final_out_d" u 1:2 w boxes fill pattern 1 lc rgb"green" title 'Accuracy', "final_out_d" u ($1+0.3):3 w boxes fill pattern 2 lc rgb"blue" title 'Earliness'

